Quantum tunneling of a single semifluxon in a 0-pi Josephson junction

We consider a symmetric 0-pi Josephson junction of length $L$, which classically can be in one of two degenerate ground states up or down, corresponding to supercurrents circulating clockwise or counterclockwise around the 0-pi boundary. When the length $L$ of the junction becomes smaller than the Josephson penetration depth $\lambda_J$, the system can switch from one state to the other due to thermal fluctuations or quantum tunneling. We map this problem to the dynamics of a single particle in a periodic double well potential and estimate parameters for which macroscopic quantum coherence may be observed. We conclude that this system is not very promising to build a qubit because (a) it requires very low temperatures to reach the quantum regime, (b) its tiny flux is hard to read out and (c) it is very sensitive to the asymmetries between the 0 and pi parts of the junction.

==> MyMc.tex <==
%%% This is 'MyMc.tex' v2.00 -- LaTeX macros for frequently used
%%% abbraviations
%%%

\RequirePackage{xspace}

%stupid macros kike \ie, \eg, \etc
\newcommand{\ie}{\textit{i.e.}\xspace}
\newcommand{\eg}{\textit{e.g.}\xspace}
\newcommand{\cf}{\textit{c.f.}\xspace}
\newcommand{\vs}{\textit{vs.}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\viz}{\textit{viz.}\xspace}
\newcommand{\etal}{\textit{et~al.}\xspace}
\newcommand{\lhs}{l.h.s.\xspace}
\newcommand{\rhs}{r.h.s.\xspace}


%units
\newcommand{\units}[1]{\ensuremath\,{\rm #1}}
%big \frac called \ratio
\newcommand{\ratio}[2]{\displaystyle\frac{#1}{#2}}
\newcommand{\fracd}[3][]{\displaystyle\frac{d^{#1}#2}{d#3^{#1}}}
\newcommand{\fracp}[3][]{\displaystyle\frac{\partial^{#1}#2}{\partial#3^{#1}}}

%Freq used materials
\newcommand{\YBCO}{YBa$_2$Cu$_3$O$_7$}

%%
%% Freq used math symbols
%%

%Elliptic fns
\newcommand{\am}{\mathop{\mathrm{am}}\nolimits}
\newcommand{\dn}{\mathop{\mathrm{dn}}\nolimits}
\newcommand{\F} {\mathop{\mathrm{F}}\nolimits}
\newcommand{\K} {\mathop{\mathrm{K}}\nolimits}
%Other fns
\newcommand{\atanh}{\mathop{\mathrm{atanh}}\nolimits}
\newcommand{\acot}{\mathop{\mathrm{acot}}\nolimits}
\newcommand{\sech}{\mathop{\mathrm{sech}}\nolimits}
\newcommand{\sgn}{\mathop{\mathrm{sgn}}\nolimits}
\newcommand{\const}{\mathop{\mathrm{const}}\nolimits}
\renewcommand{\Re}{\mathop{\mathrm{Re}}\nolimits}
\renewcommand{\Im}{\mathop{\mathrm{Im}}\nolimits}
%\newcommand{\det}{\mathop{\mathrm{det}}\nolimits}
\newcommand{\Tr}{\mathop{\mathrm{Tr}}\nolimits}

%just shortcuts
\newcommand{\HS}{\ensuremath{{\cal H}}}
\newcommand{\Heavyside}{\mathop{\mathrm{H}}\nolimits}
\newcommand{\G}{\ensuremath{{\cal G}}}
\newcommand{\Dx}{\ensuremath{{\Delta x}}}
\newcommand{\dx}{\ensuremath{{\delta x}}}
\newcommand{\Dw}{\ensuremath{{\Delta w}}}
\newcommand{\D}[1]{\ensuremath{{\Delta #1}}}
%\newcommand{\d}[1]{\ensuremath{{\delta #1}}}

%%
%% Not allowed stuff
%%
%\iffalse%{
\RequirePackage{amssymb}

%Misc. macros to discuss with co-authors
\RequirePackage{changebar}
\newcommand{\X}[1]{}
%\newcommand{\Q}[1]{\cbstart {\small\sffamily Q: #1}\cbend}
\newcommand{\Q}[1]{\par\noindent{\small\sffamily Q: #1}\par}
%\newcommand{\Q}[1]{}
\newcommand{\EG}[1]{\textcolor[rgb]{0,.7,.2}{#1}}

\newcommand{\A}[1]{\par{\small\sffamily A: #1}\par}
%
\newcommand{\KV}[1]{{\textcolor{red}{#1}}}
\newcommand{\QQ}[1]{\par\noindent{\small\sffamily \textcolor{blue}{KV: #1}}\par}


%state command which may not translate correctly
\newcommand{\stat}[1]{\state{#1}}

%%tth:\def\relax{}
%%tth:\def\message#1{}

%\tracingmacros=2
%%%%%%%%%%

\def\state#1{\ensuremath{\stt#1.}}
\def\stt#1{%
\if#1.
\let\next=\relax
\else
  \if#1u%
    \upharpoonleft%\uparrow
  \else\if#1d%
    \downharpoonleft%\downarrow
  \else\if#1U%
    \upharpoonright%\Uparrow
  \else\if#1D%
    \downharpoonright%\Downarrow
  \else\if#1F%
    \Uparrow%
  \else\if#1A%
    \Downarrow%
  \else\if#1s%
    \uparrow%
  \else\if#1a%
    \downarrow%
  \else\if#1r%
    \rightarrow%
  \else\if#1l%
    \leftarrow%
  \else\if#1R%
    \Rightarrow%
  \else\if#1L%
    \Leftarrow%
  \else\if#1>%
    \longrightarrow%
  \else\if#1<%
    \longleftarrow%
  \else\if#1%
  \relax%
  \else
  ?\message{Unknown symbol #1 in the argument of macro state}
  \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
\let\next=\stt
\fi
\next
}

\newcommand{\qstate}[1]{\ensuremath{\left\lvert\state{#1}\right\rangle}}

%\fi%}

